On the potential cosmogenic origin of the ultra-high-energy event KM3-230213A

On the 13th February 2023 the KM3NeT/ARCA telescope observed a track-like event compatible with a ultra-high-energy muon with an estimated energy of 120 PeV, produced by a neutrino with an even higher energy, making it the most energetic neutrino event ever detected. A diffuse cosmogenic component is expected to originate from the interactions of ultra-high-energy cosmic rays with ambient photon and matter fields. The flux level required by the KM3NeT/ARCA event is however in tension with the standard cosmogenic neutrino predictions based on the observations collected by the Pierre Auger Observatory and Telescope Array over the last decade of the ultra-high-energy cosmic rays above the ankle (hence from the local Universe, $z\lesssim 1$). We show here that both observations can be reconciled by extending the integration of the equivalent cosmogenic neutrino flux up to a redshift of $z\simeq 6$ and assuming a subdominant fraction of protons in the ultra-high-energy cosmic-ray flux, thus placing constraints on known cosmic accelerators.

==> authors.tex <==
\collaboration{350}{The KM3NeT Collaboration}\\
\author{S.~Aiello}
\affiliation{INFN, Sezione di Catania, (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\author{A.~Albert}
\affiliation{Universit{\'e}~de~Strasbourg,~CNRS,~IPHC~UMR~7178,~F-67000~Strasbourg,~France}
\affiliation{Universit{\'e} de Haute Alsace, rue des Fr{\`e}res Lumi{\`e}re, 68093 Mulhouse Cedex, France}
\author{A.\,R.~Alhebsi}
\affiliation{Khalifa University of Science and Technology, Department of Physics, PO Box 127788, Abu Dhabi,   United Arab Emirates}
\author{M.~Alshamsi}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{S. Alves Garre}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{A. Ambrosone}
\affiliation{Universit{\`a} di Napoli ``Federico II'', Dip. Scienze Fisiche ``E. Pancini'', Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{F.~Ameli}
\affiliation{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\author{M.~Andre}
\affiliation{Universitat Polit{\`e}cnica de Catalunya, Laboratori d'Aplicacions Bioac{\'u}stiques, Centre Tecnol{\`o}gic de Vilanova i la Geltr{\'u}, Avda. Rambla Exposici{\'o}, s/n, Vilanova i la Geltr{\'u}, 08800 Spain}
\author{L.~Aphecetche}
\affiliation{Subatech, IMT Atlantique, IN2P3-CNRS, Nantes Universit{\'e}, 4 rue Alfred Kastler - La Chantrerie, Nantes, BP 20722 44307 France}
\author{M. Ardid}
\affiliation{Universitat Polit{\`e}cnica de Val{\`e}ncia, Instituto de Investigaci{\'o}n para la Gesti{\'o}n Integrada de las Zonas Costeras, C/ Paranimf, 1, Gandia, 46730 Spain}
\author{S. Ardid}
\affiliation{Universitat Polit{\`e}cnica de Val{\`e}ncia, Instituto de Investigaci{\'o}n para la Gesti{\'o}n Integrada de las Zonas Costeras, C/ Paranimf, 1, Gandia, 46730 Spain}
\author{J.~Aublin}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{F.~Badaracco}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{L.~Bailly-Salins}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{Z. Barda\v{c}ov\'{a}}
\affiliation{Comenius University in Bratislava, Department of Nuclear Physics and Biophysics, Mlynska dolina F1, Bratislava, 842 48 Slovak Republic}
\affiliation{Czech Technical University in Prague, Institute of Experimental and Applied Physics, Husova 240/5, Prague, 110 00 Czech Republic}
\author{B.~Baret}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{A. Bariego-Quintana}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{Y.~Becherini}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{M.~Bendahman}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{F.~Benfenati~Gualandi}
\affiliation{Universit{\`a} di Bologna, Dipartimento di Fisica e Astronomia, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{M.~Benhassi}
\affiliation{Universit{\`a} degli Studi della Campania "Luigi Vanvitelli", Dipartimento di Matematica e Fisica, viale Lincoln 5, Caserta, 81100 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{M.~Bennani}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{D.\,M.~Benoit}
\affiliation{E.\,A.~Milne Centre for Astrophysics, University~of~Hull, Hull, HU6 7RX, United Kingdom}
\author{E.~Berbee}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{E.~Berti}
\affiliation{INFN, Sezione di Firenze, via Sansone 1, Sesto Fiorentino, 50019 Italy}
\author{V.~Bertin}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{P.~Betti}
\affiliation{INFN, Sezione di Firenze, via Sansone 1, Sesto Fiorentino, 50019 Italy}
\author{S.~Biagi}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{M.~Boettcher}
\affiliation{North-West University, Centre for Space Research, Private Bag X6001, Potchefstroom, 2520 South Africa}
\author{D.~Bonanno}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{S.~Bottai}
\affiliation{INFN, Sezione di Firenze, via Sansone 1, Sesto Fiorentino, 50019 Italy}
\author{J.~Boumaaza}
\affiliation{University Mohammed V in Rabat, Faculty of Sciences, 4 av.~Ibn Battouta, B.P.~1014, R.P.~10000 Rabat, Morocco}
\author{M.~Bouta}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{M.~Bouwhuis}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{C.~Bozza}
\affiliation{Universit{\`a} di Salerno e INFN Gruppo Collegato di Salerno, Dipartimento di Fisica, Via Giovanni Paolo II 132, Fisciano, 84084 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{R.\,M.~Bozza}
\affiliation{Universit{\`a} di Napoli ``Federico II'', Dip. Scienze Fisiche ``E. Pancini'', Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{H.Br\^{a}nza\c{s}}
\affiliation{ISS, Atomistilor 409, M\u{a}gurele, RO-077125 Romania}
\author{F.~Bretaudeau}
\affiliation{Subatech, IMT Atlantique, IN2P3-CNRS, Nantes Universit{\'e}, 4 rue Alfred Kastler - La Chantrerie, Nantes, BP 20722 44307 France}
\author{M.~Breuhaus}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{R.~Bruijn}
\affiliation{University of Amsterdam, Institute of Physics/IHEF, PO Box 94216, Amsterdam, 1090 GE Netherlands}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{J.~Brunner}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{R.~Bruno}
\affiliation{INFN, Sezione di Catania, (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\author{E.~Buis}
\affiliation{TNO, Technical Sciences, PO Box 155, Delft, 2600 AD Netherlands}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{R.~Buompane}
\affiliation{Universit{\`a} degli Studi della Campania "Luigi Vanvitelli", Dipartimento di Matematica e Fisica, viale Lincoln 5, Caserta, 81100 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{J.~Busto}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{B.~Caiffi}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{D.~Calvo}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{A.~Capone}
\affiliation{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation{Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\author{F.~Carenini}
\affiliation{Universit{\`a} di Bologna, Dipartimento di Fisica e Astronomia, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{V.~Carretero}
\affiliation{University of Amsterdam, Institute of Physics/IHEF, PO Box 94216, Amsterdam, 1090 GE Netherlands}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{T.~Cartraud}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{P.~Castaldi}
\affiliation{Universit{\`a} di Bologna, Dipartimento di Ingegneria dell'Energia Elettrica e dell'Informazione "Guglielmo Marconi", Via dell'Universit{\`a} 50, Cesena, 47521 Italia}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{V.~Cecchini}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{S.~Celli}
\affiliation{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation{Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\author{L.~Cerisy}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{M.~Chabab}
\affiliation{Cadi Ayyad University, Physics Department, Faculty of Science Semlalia, Av. My Abdellah, P.O.B. 2390, Marrakech, 40000 Morocco}
\author{A.~Chen}
\affiliation{University of the Witwatersrand, School of Physics, Private Bag 3, Johannesburg, Wits 2050 South Africa}
\author{S.~Cherubini}
\affiliation{Universit{\`a} di Catania, Dipartimento di Fisica e Astronomia "Ettore Majorana", (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{T.~Chiarusi}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{M.~Circella}
\affiliation{INFN, Sezione di Bari, via Orabona, 4, Bari, 70125 Italy}
\author{R.~Clark}
\affiliation{UCLouvain, Centre for Cosmology, Particle Physics and Phenomenology, Chemin du Cyclotron, 2, Louvain-la-Neuve, 1348 Belgium}
\author{R.~Cocimano}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{J.\,A.\,B.~Coelho}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{A.~Coleiro}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{A. Condorelli}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{R.~Coniglione}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{P.~Coyle}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{A.~Creusot}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{G.~Cuttone}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{R.~Dallier}
\affiliation{Subatech, IMT Atlantique, IN2P3-CNRS, Nantes Universit{\'e}, 4 rue Alfred Kastler - La Chantrerie, Nantes, BP 20722 44307 France}
\author{A.~De~Benedittis}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{G.~De~Wasseige}
\affiliation{UCLouvain, Centre for Cosmology, Particle Physics and Phenomenology, Chemin du Cyclotron, 2, Louvain-la-Neuve, 1348 Belgium}
\author{V.~Decoene}
\affiliation{Subatech, IMT Atlantique, IN2P3-CNRS, Nantes Universit{\'e}, 4 rue Alfred Kastler - La Chantrerie, Nantes, BP 20722 44307 France}
\author{P. Deguire}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{I.~Del~Rosso}
\affiliation{Universit{\`a} di Bologna, Dipartimento di Fisica e Astronomia, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{L.\,S.~Di~Mauro}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{I.~Di~Palma}
\affiliation{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation{Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\author{A.\,F.~D\'\i{}az}
\affiliation{University of Granada, Department of Computer Engineering, Automation and Robotics / CITIC, 18071 Granada, Spain}
\author{D.~Diego-Tortosa}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{C.~Distefano}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{A.~Domi}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{C.~Donzaud}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{D.~Dornic}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{E.~Drakopoulou}
\affiliation{NCSR Demokritos, Institute of Nuclear and Particle Physics, Ag. Paraskevi Attikis, Athens, 15310 Greece}
\author{D.~Drouhin}
\affiliation{Universit{\'e}~de~Strasbourg,~CNRS,~IPHC~UMR~7178,~F-67000~Strasbourg,~France}
\affiliation{Universit{\'e} de Haute Alsace, rue des Fr{\`e}res Lumi{\`e}re, 68093 Mulhouse Cedex, France}
\author{J.-G. Ducoin}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{P.~Duverne}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{R. Dvornick\'{y}}
\affiliation{Comenius University in Bratislava, Department of Nuclear Physics and Biophysics, Mlynska dolina F1, Bratislava, 842 48 Slovak Republic}
\author{T.~Eberl}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{E. Eckerov\'{a}}
\affiliation{Comenius University in Bratislava, Department of Nuclear Physics and Biophysics, Mlynska dolina F1, Bratislava, 842 48 Slovak Republic}
\affiliation{Czech Technical University in Prague, Institute of Experimental and Applied Physics, Husova 240/5, Prague, 110 00 Czech Republic}
\author{A.~Eddymaoui}
\affiliation{University Mohammed V in Rabat, Faculty of Sciences, 4 av.~Ibn Battouta, B.P.~1014, R.P.~10000 Rabat, Morocco}
\author{T.~van~Eeden}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{M.~Eff}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{D.~van~Eijk}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{I.~El~Bojaddaini}
\affiliation{University Mohammed I, Faculty of Sciences, BV Mohammed VI, B.P.~717, R.P.~60000 Oujda, Morocco}
\author{S.~El~Hedri}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{S.~El~Mentawi}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{V.~Ellajosyula}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{A.~Enzenh\"ofer}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{G.~Ferrara}
\affiliation{Universit{\`a} di Catania, Dipartimento di Fisica e Astronomia "Ettore Majorana", (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{M.~D.~Filipovi\'c}
\affiliation{Western Sydney University, School of Computing, Engineering and Mathematics, Locked Bag 1797, Penrith, NSW 2751 Australia}
\author{F.~Filippini}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{D.~Franciotti}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{L.\,A.~Fusco}
\affiliation{Universit{\`a} di Salerno e INFN Gruppo Collegato di Salerno, Dipartimento di Fisica, Via Giovanni Paolo II 132, Fisciano, 84084 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{S.~Gagliardini}
\affiliation{Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\author{T.~Gal}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{J.~Garc{\'\i}a~M{\'e}ndez}
\affiliation{Universitat Polit{\`e}cnica de Val{\`e}ncia, Instituto de Investigaci{\'o}n para la Gesti{\'o}n Integrada de las Zonas Costeras, C/ Paranimf, 1, Gandia, 46730 Spain}
\author{A.~Garcia~Soto}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{C.~Gatius~Oliver}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{N.~Gei{\ss}elbrecht}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{E.~Genton}
\affiliation{UCLouvain, Centre for Cosmology, Particle Physics and Phenomenology, Chemin du Cyclotron, 2, Louvain-la-Neuve, 1348 Belgium}
\author{H.~Ghaddari}
\affiliation{University Mohammed I, Faculty of Sciences, BV Mohammed VI, B.P.~717, R.P.~60000 Oujda, Morocco}
\author{L.~Gialanella}
\affiliation{Universit{\`a} degli Studi della Campania "Luigi Vanvitelli", Dipartimento di Matematica e Fisica, viale Lincoln 5, Caserta, 81100 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{B.\,K.~Gibson}
\affiliation{E.\,A.~Milne Centre for Astrophysics, University~of~Hull, Hull, HU6 7RX, United Kingdom}
\author{E.~Giorgio}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{I.~Goos}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{P.~Goswami}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{S.\,R.~Gozzini}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{R.~Gracia}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{C.~Guidi}
\affiliation{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{B.~Guillon}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{M.~Guti{\'e}rrez}
\affiliation{University of Granada, Dpto.~de F\'\i{}sica Te\'orica y del Cosmos \& C.A.F.P.E., 18071 Granada, Spain}
\author{C.~Haack}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{H.~van~Haren}
\affiliation{NIOZ (Royal Netherlands Institute for Sea Research), PO Box 59, Den Burg, Texel, 1790 AB, the Netherlands}
\author{A.~Heijboer}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{L.~Hennig}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{J.\,J.~Hern{\'a}ndez-Rey}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{A.~Idrissi}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{W.~Idrissi~Ibnsalih}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{G.~Illuminati}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{O.~Janik}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{D.~Joly}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{M.~de~Jong}
\affiliation{Leiden University, Leiden Institute of Physics, PO Box 9504, Leiden, 2300 RA Netherlands}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{P.~de~Jong}
\affiliation{University of Amsterdam, Institute of Physics/IHEF, PO Box 94216, Amsterdam, 1090 GE Netherlands}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{B.\,J.~Jung}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{P.~Kalaczy\'nski}
\affiliation{AstroCeNT, Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, Rektorska 4, Warsaw, 00-614 Poland}
\affiliation{AGH University of Krakow, Al.~Mickiewicza 30, 30-059 Krakow, Poland}
\author{J.~Keegans}
\affiliation{E.\,A.~Milne Centre for Astrophysics, University~of~Hull, Hull, HU6 7RX, United Kingdom}
\author{V.~Kikvadze}
\affiliation{Tbilisi State University, Department of Physics, 3, Chavchavadze Ave., Tbilisi, 0179 Georgia}
\author{G.~Kistauri}
\affiliation{The University of Georgia, Institute of Physics, Kostava str. 77, Tbilisi, 0171 Georgia}
\affiliation{Tbilisi State University, Department of Physics, 3, Chavchavadze Ave., Tbilisi, 0179 Georgia}
\author{C.~Kopper}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{A.~Kouchner}
\affiliation{Institut Universitaire de France, 1 rue Descartes, Paris, 75005 France}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{Y. Y. Kovalev}
\affiliation{Max-Planck-Institut~f{\"u}r~Radioastronomie,~Auf~dem H{\"u}gel~69,~53121~Bonn,~Germany}
\author{L.~Krupa}
\affiliation{Czech Technical University in Prague, Institute of Experimental and Applied Physics, Husova 240/5, Prague, 110 00 Czech Republic}
\author{V.~Kueviakoe}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{V.~Kulikovskiy}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{R.~Kvatadze}
\affiliation{The University of Georgia, Institute of Physics, Kostava str. 77, Tbilisi, 0171 Georgia}
\author{M.~Labalme}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{R.~Lahmann}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{M.~Lamoureux}
\affiliation{UCLouvain, Centre for Cosmology, Particle Physics and Phenomenology, Chemin du Cyclotron, 2, Louvain-la-Neuve, 1348 Belgium}
\author{G.~Larosa}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{C.~Lastoria}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{J.~Lazar}
\affiliation{UCLouvain, Centre for Cosmology, Particle Physics and Phenomenology, Chemin du Cyclotron, 2, Louvain-la-Neuve, 1348 Belgium}
\author{A.~Lazo}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{S.~Le~Stum}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{G.~Lehaut}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{V.~Lema{\^\i}tre}
\affiliation{UCLouvain, Centre for Cosmology, Particle Physics and Phenomenology, Chemin du Cyclotron, 2, Louvain-la-Neuve, 1348 Belgium}
\author{E.~Leonora}
\affiliation{INFN, Sezione di Catania, (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\author{N.~Lessing}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{G.~Levi}
\affiliation{Universit{\`a} di Bologna, Dipartimento di Fisica e Astronomia, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{M.~Lindsey~Clark}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{F.~Longhitano}
\affiliation{INFN, Sezione di Catania, (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\author{F.~Magnani}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{J.~Majumdar}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{L.~Malerba}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{F.~Mamedov}
\affiliation{Czech Technical University in Prague, Institute of Experimental and Applied Physics, Husova 240/5, Prague, 110 00 Czech Republic}
\author{A.~Manfreda}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{A.~Manousakis}
\affiliation{University of Sharjah, Sharjah Academy for Astronomy, Space Sciences, and Technology, University Campus - POB 27272, Sharjah, - United Arab Emirates}
\author{M.~Marconi}
\affiliation{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{A.~Margiotta}
\affiliation{Universit{\`a} di Bologna, Dipartimento di Fisica e Astronomia, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{A.~Marinelli}
\affiliation{Universit{\`a} di Napoli ``Federico II'', Dip. Scienze Fisiche ``E. Pancini'', Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{C.~Markou}
\affiliation{NCSR Demokritos, Institute of Nuclear and Particle Physics, Ag. Paraskevi Attikis, Athens, 15310 Greece}
\author{L.~Martin}
\affiliation{Subatech, IMT Atlantique, IN2P3-CNRS, Nantes Universit{\'e}, 4 rue Alfred Kastler - La Chantrerie, Nantes, BP 20722 44307 France}
\author{M.~Mastrodicasa}
\affiliation{Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\author{S.~Mastroianni}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{J.~Mauro}
\affiliation{UCLouvain, Centre for Cosmology, Particle Physics and Phenomenology, Chemin du Cyclotron, 2, Louvain-la-Neuve, 1348 Belgium}
\author{K.\,C.\,K.~Mehta}
\affiliation{AGH University of Krakow, Al.~Mickiewicza 30, 30-059 Krakow, Poland}
\author{A.~Meskar}
\affiliation{National~Centre~for~Nuclear~Research,~02-093~Warsaw,~Poland}
\author{G.~Miele}
\affiliation{Universit{\`a} di Napoli ``Federico II'', Dip. Scienze Fisiche ``E. Pancini'', Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{P.~Migliozzi}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{E.~Migneco}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{M.\,L.~Mitsou}
\affiliation{Universit{\`a} degli Studi della Campania "Luigi Vanvitelli", Dipartimento di Matematica e Fisica, viale Lincoln 5, Caserta, 81100 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{C.\,M.~Mollo}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{L. Morales-Gallegos}
\affiliation{Universit{\`a} degli Studi della Campania "Luigi Vanvitelli", Dipartimento di Matematica e Fisica, viale Lincoln 5, Caserta, 81100 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}

\author{N.~Mori}
\affiliation{INFN, Sezione di Firenze, via Sansone 1, Sesto Fiorentino, 50019 Italy}

\author{A.~Moussa}
\affiliation{University Mohammed I, Faculty of Sciences, BV Mohammed VI, B.P.~717, R.P.~60000 Oujda, Morocco}
\author{I.~Mozun~Mateo}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{R.~Muller}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{M.\,R.~Musone}
\affiliation{Universit{\`a} degli Studi della Campania "Luigi Vanvitelli", Dipartimento di Matematica e Fisica, viale Lincoln 5, Caserta, 81100 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{M.~Musumeci}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{S.~Navas}
\affiliation{University of Granada, Dpto.~de F\'\i{}sica Te\'orica y del Cosmos \& C.A.F.P.E., 18071 Granada, Spain}
\author{A.~Nayerhoda}
\affiliation{INFN, Sezione di Bari, via Orabona, 4, Bari, 70125 Italy}
\author{C.\,A.~Nicolau}
\affiliation{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\author{B.~Nkosi}
\affiliation{University of the Witwatersrand, School of Physics, Private Bag 3, Johannesburg, Wits 2050 South Africa}
\author{B.~{\'O}~Fearraigh}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{V.~Oliviero}
\affiliation{Universit{\`a} di Napoli ``Federico II'', Dip. Scienze Fisiche ``E. Pancini'', Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{A.~Orlando}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{E.~Oukacha}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{L.~Pacini}
\affiliation{INFN, Sezione di Firenze, via Sansone 1, Sesto Fiorentino, 50019 Italy}
\author{D.~Paesani}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{J.~Palacios~Gonz{\'a}lez}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{G.~Papalashvili}
\affiliation{INFN, Sezione di Bari, via Orabona, 4, Bari, 70125 Italy}
\affiliation{Tbilisi State University, Department of Physics, 3, Chavchavadze Ave., Tbilisi, 0179 Georgia}
\author{P.~Papini}
\affiliation{INFN, Sezione di Firenze, via Sansone 1, Sesto Fiorentino, 50019 Italy}
\author{V.~Parisi}
\affiliation{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{A.~Parmar}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{E.J. Pastor Gomez}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{C.~Pastore}
\affiliation{INFN, Sezione di Bari, via Orabona, 4, Bari, 70125 Italy}
\author{A.~M.~P{\u a}un}
\affiliation{ISS, Atomistilor 409, M\u{a}gurele, RO-077125 Romania}
\author{G.\,E.~P\u{a}v\u{a}la\c{s}}
\affiliation{ISS, Atomistilor 409, M\u{a}gurele, RO-077125 Romania}
\author{S. Pe\~{n}a Mart\'inez}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{M.~Perrin-Terrin}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\author{V.~Pestel}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{R.~Pestes}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{P.~Piattelli}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{A.~Plavin}
\affiliation{Max-Planck-Institut~f{\"u}r~Radioastronomie,~Auf~dem H{\"u}gel~69,~53121~Bonn,~Germany}
\affiliation{Harvard University, Black Hole Initiative, 20 Garden Street, Cambridge, MA 02138 USA}
\author{C.~Poir{\`e}}
\affiliation{Universit{\`a} di Salerno e INFN Gruppo Collegato di Salerno, Dipartimento di Fisica, Via Giovanni Paolo II 132, Fisciano, 84084 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{V.~Popa}
\affiliation{ISS, Atomistilor 409, M\u{a}gurele, RO-077125 Romania}
\author{T.~Pradier}
\affiliation{Universit{\'e}~de~Strasbourg,~CNRS,~IPHC~UMR~7178,~F-67000~Strasbourg,~France}
\author{J.~Prado}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{S.~Pulvirenti}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{C.A.~Quiroz-Rangel}
\affiliation{Universitat Polit{\`e}cnica de Val{\`e}ncia, Instituto de Investigaci{\'o}n para la Gesti{\'o}n Integrada de las Zonas Costeras, C/ Paranimf, 1, Gandia, 46730 Spain}
\author{N.~Randazzo}
\affiliation{INFN, Sezione di Catania, (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\author{A.~Ratnani}
\affiliation{School of Applied and Engineering Physics, Mohammed VI Polytechnic University, Ben Guerir, 43150, Morocco}
\author{S.~Razzaque}
\affiliation{University of Johannesburg, Department Physics, PO Box 524, Auckland Park, 2006 South Africa}
\author{I.\,C.~Rea}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{D.~Real}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{G.~Riccobene}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{J.~Robinson}
\affiliation{North-West University, Centre for Space Research, Private Bag X6001, Potchefstroom, 2520 South Africa}
\author{A.~Romanov}
\affiliation{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{E.~Ros}
\affiliation{Max-Planck-Institut~f{\"u}r~Radioastronomie,~Auf~dem H{\"u}gel~69,~53121~Bonn,~Germany}
\author{A. \v{S}aina}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{F.~Salesa~Greus}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{D.\,F.\,E.~Samtleben}
\affiliation{Leiden University, Leiden Institute of Physics, PO Box 9504, Leiden, 2300 RA Netherlands}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{A.~S{\'a}nchez~Losa}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{S.~Sanfilippo}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{M.~Sanguineti}
\affiliation{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{D.~Santonocito}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{P.~Sapienza}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{M.~Scaringella}
\affiliation{INFN, Sezione di Firenze, via Sansone 1, Sesto Fiorentino, 50019 Italy}
\author{M.~Scarnera}
\affiliation{UCLouvain, Centre for Cosmology, Particle Physics and Phenomenology, Chemin du Cyclotron, 2, Louvain-la-Neuve, 1348 Belgium}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{J.~Schnabel}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{J.~Schumann}
\affiliation{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg (FAU), Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Stra{\ss}e 2, 91058 Erlangen, Germany}
\author{H.~M. Schutte}
\affiliation{North-West University, Centre for Space Research, Private Bag X6001, Potchefstroom, 2520 South Africa}
\author{J.~Seneca}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{N.~Sennan}
\affiliation{University Mohammed I, Faculty of Sciences, BV Mohammed VI, B.P.~717, R.P.~60000 Oujda, Morocco}
\author{P.~Sevle}
\affiliation{UCLouvain, Centre for Cosmology, Particle Physics and Phenomenology, Chemin du Cyclotron, 2, Louvain-la-Neuve, 1348 Belgium}
\author{I.~Sgura}
\affiliation{INFN, Sezione di Bari, via Orabona, 4, Bari, 70125 Italy}
\author{R.~Shanidze}
\affiliation{Tbilisi State University, Department of Physics, 3, Chavchavadze Ave., Tbilisi, 0179 Georgia}
\author{A.~Sharma}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{Y.~Shitov}
\affiliation{Czech Technical University in Prague, Institute of Experimental and Applied Physics, Husova 240/5, Prague, 110 00 Czech Republic}
\author{F. \v{S}imkovic}
\affiliation{Comenius University in Bratislava, Department of Nuclear Physics and Biophysics, Mlynska dolina F1, Bratislava, 842 48 Slovak Republic}
\author{A.~Simonelli}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{A.~Sinopoulou}
\affiliation{INFN, Sezione di Catania, (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\author{B.~Spisso}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{M.~Spurio}
\affiliation{Universit{\`a} di Bologna, Dipartimento di Fisica e Astronomia, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\affiliation{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\author{O.~Starodubtsev}
\affiliation{INFN, Sezione di Firenze, via Sansone 1, Sesto Fiorentino, 50019 Italy}
\author{D.~Stavropoulos}
\affiliation{NCSR Demokritos, Institute of Nuclear and Particle Physics, Ag. Paraskevi Attikis, Athens, 15310 Greece}
\author{I. \v{S}tekl}
\affiliation{Czech Technical University in Prague, Institute of Experimental and Applied Physics, Husova 240/5, Prague, 110 00 Czech Republic}
\author{D.~Stocco}
\affiliation{Subatech, IMT Atlantique, IN2P3-CNRS, Nantes Universit{\'e}, 4 rue Alfred Kastler - La Chantrerie, Nantes, BP 20722 44307 France}
\author{M.~Taiuti}
\affiliation{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{G.~Takadze}
\affiliation{Tbilisi State University, Department of Physics, 3, Chavchavadze Ave., Tbilisi, 0179 Georgia}
\author{Y.~Tayalati}
\affiliation{University Mohammed V in Rabat, Faculty of Sciences, 4 av.~Ibn Battouta, B.P.~1014, R.P.~10000 Rabat, Morocco}
\affiliation{School of Applied and Engineering Physics, Mohammed VI Polytechnic University, Ben Guerir, 43150, Morocco}
\author{H.~Thiersen}
\affiliation{North-West University, Centre for Space Research, Private Bag X6001, Potchefstroom, 2520 South Africa}
\author{S.~Thoudam}
\affiliation{Khalifa University of Science and Technology, Department of Physics, PO Box 127788, Abu Dhabi,   United Arab Emirates}
\author{I.~Tosta~e~Melo}
\affiliation{INFN, Sezione di Catania, (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\affiliation{Universit{\`a} di Catania, Dipartimento di Fisica e Astronomia "Ettore Majorana", (INFN-CT) Via Santa Sofia 64, Catania, 95123 Italy}
\author{B.~Trocm{\'e}}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{V.~Tsourapis}
\affiliation{NCSR Demokritos, Institute of Nuclear and Particle Physics, Ag. Paraskevi Attikis, Athens, 15310 Greece}
\author{A. Tudorache}
\affiliation{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation{Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\author{E.~Tzamariudaki}
\affiliation{NCSR Demokritos, Institute of Nuclear and Particle Physics, Ag. Paraskevi Attikis, Athens, 15310 Greece}
\author{A.~Ukleja}
\affiliation{National~Centre~for~Nuclear~Research,~02-093~Warsaw,~Poland}
\affiliation{AGH University of Krakow, Al.~Mickiewicza 30, 30-059 Krakow, Poland}
\author{A.~Vacheret}
\affiliation{LPC CAEN, Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, 6 boulevard Mar{\'e}chal Juin, Caen, 14050 France}
\author{V.~Valsecchi}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{V.~Van~Elewyck}
\affiliation{Institut Universitaire de France, 1 rue Descartes, Paris, 75005 France}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{G.~Vannoye}
\affiliation{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{G.~Vasileiadis}
\affiliation{Laboratoire Univers et Particules de Montpellier, Place Eug{\`e}ne Bataillon - CC 72, Montpellier C{\'e}dex 05, 34095 France}
\author{F.~Vazquez~de~Sola}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{A. Veutro}
\affiliation{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation{Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\author{S.~Viola}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{D.~Vivolo}
\affiliation{Universit{\`a} degli Studi della Campania "Luigi Vanvitelli", Dipartimento di Matematica e Fisica, viale Lincoln 5, Caserta, 81100 Italy}
\affiliation{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\author{A. van Vliet}
\affiliation{Khalifa University of Science and Technology, Department of Physics, PO Box 127788, Abu Dhabi,   United Arab Emirates}
\author{E.~de~Wolf}
\affiliation{University of Amsterdam, Institute of Physics/IHEF, PO Box 94216, Amsterdam, 1090 GE Netherlands}
\affiliation{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\author{I.~Lhenry-Yvon}
\affiliation{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\author{S.~Zavatarelli}
\affiliation{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\author{A.~Zegarelli}
\affiliation{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation{Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\author{D.~Zito}
\affiliation{INFN, Laboratori Nazionali del Sud, (LNS) Via S. Sofia 62, Catania, 95123 Italy}
\author{J.\,D.~Zornoza}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{J.~Z{\'u}{\~n}iga}
\affiliation{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\author{N.~Zywucka}
\affiliation{North-West University, Centre for Space Research, Private Bag X6001, Potchefstroom, 2520 South Africa}
